Facebook AI's WAT19 Myanmar-English Translation Task Submission

This paper describes Facebook AI's submission to the WAT 2019 Myanmar-English translation task. Our baseline systems are BPE-based transformer models. We explore methods to leverage monolingual data to improve generalization, including self-training, back-translation and their combination. We further improve results by using noisy channel re-ranking and ensembling. We demonstrate that these techniques can significantly improve not only a system trained with additional monolingual data, but even the baseline system trained exclusively on the provided small parallel dataset. Our system ranks first in both directions according to human evaluation and BLEU, with a gain of over 8 BLEU points above the second best system.

==> backtranslation.tex <==
\subsection{Back-Translation (BT)}
\label{sec:back_translation}
Back-translation~\citep{sennrich2015improving} is an effective data augmentation method  leveraging target side monolingual data. To perform back-translation, we first train a backward model and use it to translate the target side monolingual data to source side synthetic  data. We follow the TaggedBT approach \citep{caswell2019tagged} to combine the bitext data and the back-translated data, where each back-translated sentence in the source language is prepended with a $\langle BT \rangle$ tag. We then concatenate the bitext data with the back-translated data and train the forward translation model from scratch. The upsampling ratio of the bitext data is optimized together with the other hyper-parameters on the validation set.

We compare two decoding strategies, beam-search decoding and noisy channel decoding, when generating back-translated data. We use beam size 5 for beam-search decoding and the same setting as \textsection\ref{sec:noisy_channel} for noisy channel decoding. Our experiments in Table~ \ref{tab:noisy_channel_bt}  show that  back-translated data decoded by noisy channel reranking yields better BLEU score. \vc{It seems like we used Tagged BT as a default. Do we have numbers without tagged BT ? From the table it seems like Tagged BT is only used in row 1?}

\begin{table}[t]
\centering
\begin{tabular}{l r r}
\hline
Model & My$\rightarrow$En & En$\rightarrow$My \\
Iteration 1 Tagged-BT \\\hline
Beam-5 & 30.32 & 38.19\\
Noisy channel re-ranked & 32.45 & 38.92\\\hline
\end{tabular}
\caption{\label{tab:noisy_channel_bt} BLEU scores of a model trained with back-translated data which has been decoded using either beam or noisy channel reranking.}
\end{table}

\subsection{Self-Training (ST)}
Self-training~\citep{yarowski,ueffing, zhang16} is another way to augment the original parallel dataset. This augments the original parallel dataset with synthetic pairs 
composed by a sentence from the source monolingual dataset with the corresponding forward model translation as target.
The potential advantage of this method is that the source side monolingual data can be more in-domain with the test set, which is certainly the case for the English to Myanmar direction. The shortcoming is that targets are often incorrect and may deteriorate performance.
To indicate to the model that the data comes from self-training and allow the model to treat it as a different domain, we prepend the source sentence with a $\langle ST \rangle$ tag. We then upsample the bitext data, concatenate it with the self-trained data and train the forward model from scratch. We also use noisy channel decoding when generating self-trained data as discussed in \textsection\ref{sec:noisy_channel} and \textsection\ref{sec:back_translation}.

Self-training and back-translation are complementary to each other. One is better when the source monolingual data is in-domain while the latter is better when the target monolingual data is in-domain, relative to the domain of the test set. Moreover, self-training trades off the potential gains coming from learning from in-domain data with the potential loss due to the noise in the synthetic references.

In our experiments, we combine bitext data together with self-trained and back-translated data. The upsample ratios for each dataset are tuned via hyper-parameter search on the validation set. The experiment reported in Table \ref{tab:self_training} shows that the combined approach yields better performance than each individual method. \vc{If we are just using Noisy Channel reranking for BT as well, let's specify it here}

\begin{table}[t]
\centering
\begin{tabular}{l r r}
\hline
Model & My$\rightarrow$En & En$\rightarrow$My \\\hline
Tagged BT & 33.05 & 39.54\\
Tagged ST & 33.21 & 39.92\\
Tagged BT + Tagged ST & 34.14 & 40.28\\\hline
\end{tabular}
\caption{\label{tab:self_training}
Combining self-training and back-translation improves performance in both directions.
}
\end{table}

\subsection{Final Iterative Algorithm} \label{sec:iterative}
The final algorithm proceeds in rounds. At each round, we are provided with a forward model and a backward model. The forward model is used to forward translated source  monolingual data (possibly via noisy channel reranking)\vc{Why do we say possibly here ? In 3.3 we say that we use Noisy Channel for ST}. This is going to be used as self-trained data to improve the forward model, and as back-translated data to improve the backward model. Similarly, the backward model is used to back-translate target monolingual data (possibly via noisy channel reranking). This data is then used to improve the forward model via back-translation, but also the backward model via self-training.

To summarize, at each iteration we use the forward and backward models to translate monolingual data on the source and target side, respectively. We then concatenate the original parallel dataset (up to a certain up-sampling ratio) with the forward and back-translated data. We then use this data to retrain both forward and backward models (the latter with the roles of source and target language simply swapped). This whole process of generation and training then repeats as many times as desired.

\begin{algorithm}[t]
\SetAlgoLined
\footnotesize
\nl \KwData{Given a parallel dataset $\{X,Y\}$, a source monolingual dataset $\mathcal{M_S}$ and a target monolingual dataset $\mathcal{M_T}$\;}
\nl Given an initial forward model $\overrightarrow{f}$ and backward model $\overleftarrow{g}$\;
\nl Let $N$ be the number of hyper-parameter configurations tested during grid search training\;
\nl Let $k$ be the number of models used in the ensemble\;
  \nl \For{$t$ \textbf{in} $[1 \dots T]$}{
    \nl forward-translated data: $\mathcal{F} \longleftarrow \overrightarrow{f}(\mathcal{M_S})$\;
    \nl back-translated data: $\mathcal{B} \longleftarrow \overleftarrow{g}(\mathcal{M_T})$\; 
    \nl $\{\overrightarrow{f}_i\}_{i=1 \dots N} \longleftarrow$ grid search using: $\{X,Y\} \cup \{\mathcal{M_S}, \mathcal{F} \} \cup \{\mathcal{B}, \mathcal{M_T} \}$\; 
    \nl $\{\overleftarrow{g}_i\}_{i=1 \dots N} \longleftarrow$
    \nl grid search using: $\{Y,X\} \cup \{\mathcal{F}, \mathcal{M_S} \} \cup \{\mathcal{M_T}, \mathcal{B} \}$\; 
    \nl \If{t == T}{ 
       \nl Fine-tune $\{\overrightarrow{f}_i\}_{i=1 \dots N}$ and $\{\overleftarrow{g}_i\}_{i=1 \dots N}$  on the in-domain ALT dataset\; 
    }
    \nl $\overrightarrow{f}$ $\longleftarrow$ ensemble of top k best models from $\{\overrightarrow{f}_i\}_{i=1 \dots N}$\; 
    \nl $\overleftarrow{g}$ $\longleftarrow$ ensemble of top k best models from $\{\overleftarrow{g}_i\}_{i=1 \dots N}$\; 
  }
 \KwResult{Forward MT system $\overrightarrow{f}$ and backward MT system $\overleftarrow{g}$}
\caption{Iterative Learning Algorithm\label{algo:iterativeSTBT}}
\end{algorithm}


==> finetuning_ensemble.tex <==
\subsection{Fine-tuning and Ensembling}

We applied fine-tuning to the supervised baseline models and models in final iteration. Fine-tuning is common and effective way to adapt to the test  domain. In our case, since the test examples are from the ALT corpus, we fine-tune the model on the ALT training data 
once the iterative process described in \textsection\ref{sec:iterative} is terminated.

Empirically we found that ensembling always increases BLEU by about 1 BLEU point \mr{please correct this, is it possible to quantify the gain?}. All our intermediate models, including the models we used to generate self-trained and back-translated data as well as forward and backward models  used for noisy channel reranking, are ensembles of N fine-tuned models. \mr{what is N?} \vc{Also if we are using fine-tuned models, we should explain fine-tuning before this portion}




==> noisy_channel.tex <==
\subsection{Noisy Channel Model Reranking (NC)}\label{sec:noisy_channel}
Noisy channel model reranking~\citep{noisychannel} is an approach to better select a candidate hypothesis by reranking the $n$-best hypotheses generated by beam search scoring. It has been used by the winning submissions of the WMT2019 news translation shared task for English-German, German-English, English-Russian and Russian-English~\citep{ng2019facebook}, and here we followed the same methodology.

More specifically, given a source sequence $x$ and a target sequence $y$, we compute the following score:
\begin{equation}
\log P(y|x) + \lambda_1 \log P(x|y) + \lambda_2 \log P(y) \label{eq:nc}
\end{equation}
where $\log P(y|x)$, $\log P(x|y)$ and $\log P(y)$ are the forward model, backward model and language model scores. The score can be used to rerank the $n$-best target hypotheses for each source sequence and the highest ranked hypothesis is selected. In our experiments we set $n$ to 50. The weights $\lambda_1$ and $\lambda_2$ are tuned via random search on the validation set.

We apply noisy channel reranking in the last step of each  iteration, see \textsection\ref{sec:iterative} \mr{what is a step here? Maybe we should say that we apply it when we generate either self-training or back-translation data?}. We choose the forward model yielding the highest validation BLEU \mr{i do not understand what you want to say here. We already discussed how we select models, no?}. This model is also used as backward model for the reverse direction \mr{this seems out of place}. Our language models are also based on the transformer architecture. While the English language model is trained on the common crawl news dataset, the Burmese language model is trained on the common crawl dataset and fine-tuned on the ALT training set. For the submission which does not make use of additional data, smaller transformer language models were trained on each side of the provided parallel corpus. \mr{This paragraph needs revision.}

For both directions, we observed gains when applying noisy channel reranking, as shown in Table~\ref{tab:noisy_channel}.

\begin{table}[t]
\centering
\begin{tabular}{l r r}
\hline
Model & My$\rightarrow$En & En$\rightarrow$My \\\hline
baseline & 25.1 & 35.92\\
+reranking (w/o mono) & 26.32 & 36.78\\
baseline with BT (w/ mono) & 30.32 & 38.19\\
+reranking (w/ mono) & 35.62 & 39.37\\\hline
\end{tabular}
\caption{Effect of noisy channel reranking over baseline models trained on the provided parallel dataset.} \label{tab:noisy_channel}
\end{table}




==> selftranslation.tex <==
\subsection{Self-Training (ST)}
Self-training~\citep{yarowski,ueffing, zhang16} is another way to augment the original parallel dataset. This augments the original parallel dataset with synthetic pairs 
composed by a sentence from the source monolingual dataset with the corresponding forward model translation as target.
The potential advantage of this method is that the source side monolingual data can be more in-domain with the test set, which is certainly the case for the English to Myanmar direction. The shortcoming is that targets are often incorrect and may deteriorate performance.
To indicate to the model that the data comes from self-training and allow the model to treat it as a different domain, we prepend the source sentence with a $\langle ST \rangle$ tag. We then upsample the bitext data, concatenate it with the self-trained data and train the forward model from scratch. We also use noisy channel decoding when generating self-trained data as discussed in \textsection\ref{sec:noisy_channel} and \textsection\ref{sec:back_translation}.

Self-training and back-translation are complementary to each other. One is better when the source monolingual data is in-domain while the latter is better when the target monolingual data is in-domain, relative to the domain of the test set. Moreover, self-training trades off the potential gains coming from learning from in-domain data with the potential loss due to the noise in the synthetic references.

In our experiments, we combine bitext data together with self-trained and back-translated data. The upsample ratios for each dataset are tuned via hyper-parameter search on the validation set. The experiment reported in Table \ref{tab:self_training} shows that the combined approach yields better performance than each individual method. \vc{If we are just using Noisy Channel reranking for BT as well, let's specify it here}

\begin{table}[t]
\centering
\begin{tabular}{l | c |  c}
\hline
Model & My$\rightarrow$En & En$\rightarrow$My \\\hline
Tagged BT & 33.1 & 39.5\\
Tagged ST & 33.2 & 39.9\\
Tagged BT + Tagged ST & 34.1 & 40.3\\\hline
\end{tabular}
\caption{\label{tab:self_training}
Combining self-training and back-translation improves performance in both directions.
}
\end{table}

\subsection{Final Iterative Algorithm} \label{sec:iterative}
The final algorithm proceeds in rounds. At each round, we are provided with a forward model and a backward model. The forward model is used to forward translated source  monolingual data (possibly via noisy channel reranking)\vc{Why do we say possibly here ? In 3.3 we say that we use Noisy Channel for ST}. This is going to be used as self-trained data to improve the forward model, and as back-translated data to improve the backward model. Similarly, the backward model is used to back-translate target monolingual data (possibly via noisy channel reranking). This data is then used to improve the forward model via back-translation, but also the backward model via self-training.

To summarize, at each iteration we use the forward and backward models to translate monolingual data on the source and target side, respectively. We then concatenate the original parallel dataset (up to a certain up-sampling ratio) with the forward and back-translated data. We then use this data to retrain both forward and backward models (the latter with the roles of source and target language simply swapped). This whole process of generation and training then repeats as many times as desired.

\begin{algorithm}[t]
\SetAlgoLined
\footnotesize
\nl \KwData{Given a parallel dataset $\{X,Y\}$, a source monolingual dataset $\mathcal{M_S}$ and a target monolingual dataset $\mathcal{M_T}$\;}
\nl Given an initial forward model $\overrightarrow{f}$ and backward model $\overleftarrow{g}$\;
\nl Let $N$ be the number of hyper-parameter configurations tested during grid search training\;
\nl Let $k$ be the number of models used in the ensemble\;
  \nl \For{$t$ \textbf{in} $[1 \dots T]$}{
    \nl forward-translated data: $\mathcal{F} \longleftarrow \overrightarrow{f}(\mathcal{M_S})$\;
    \nl back-translated data: $\mathcal{B} \longleftarrow \overleftarrow{g}(\mathcal{M_T})$\; 
    \nl $\{\overrightarrow{f}_i\}_{i=1 \dots N} \longleftarrow$ grid search using: $\{X,Y\} \cup \{\mathcal{M_S}, \mathcal{F} \} \cup \{\mathcal{B}, \mathcal{M_T} \}$\; 
    \nl $\{\overleftarrow{g}_i\}_{i=1 \dots N} \longleftarrow$
    \nl grid search using: $\{Y,X\} \cup \{\mathcal{F}, \mathcal{M_S} \} \cup \{\mathcal{M_T}, \mathcal{B} \}$\; 
    \nl \If{t == T}{ 
       \nl Fine-tune $\{\overrightarrow{f}_i\}_{i=1 \dots N}$ and $\{\overleftarrow{g}_i\}_{i=1 \dots N}$  on the in-domain ALT dataset\; 
    }
    \nl $\overrightarrow{f}$ $\longleftarrow$ ensemble of top k best models from $\{\overrightarrow{f}_i\}_{i=1 \dots N}$\; 
    \nl $\overleftarrow{g}$ $\longleftarrow$ ensemble of top k best models from $\{\overleftarrow{g}_i\}_{i=1 \dots N}$\; 
  }
 \KwResult{Forward MT system $\overrightarrow{f}$ and backward MT system $\overleftarrow{g}$}
\caption{Iterative Learning Algorithm\label{algo:iterativeSTBT}}
\end{algorithm}

